The Model Forest Ensemble Kalman Filter

Traditional data assimilation uses information obtained from the propagation of one physics-driven model and combines it with information derived from real-world observations in order to obtain a better estimate of the truth of some natural process. However, in many situations multiple simulation models that describe the same physical phenomenon are available. Such models can have different sources. On one hand there are theory-guided models are constructed from first physical principles, while on the other there are data-driven models that are constructed from snapshots of high fidelity information. In this work we provide a possible way to make use of this collection of models in data assimilation by generalizing the idea of model hierarchies into model forests -- collections of high fidelity and low fidelity models organized in a groping of model trees such as to capture various relationships between different models. We generalize the multifidelity ensemble Kalman filter that previously operated on model hierarchies into the model forest ensemble Kalman filter through a generalized theory of linear control variates. This new filter allows for much more freedom when treading the line between accuracy and speed. Numerical experiments with a high fidelity quasi-geostrophic model and two of its low fidelity reduced order models validate the accuracy of our approach.

==> Model Forest EnKF_1_sub/header.tex <==
%\usepackage[dvips]{graphics}
%\usepackage[pdftex]{graphics}
%\newcommand\hmmax{0}
%\newcommand\bmmax{0}
%\usepackage{bbm,mathrsfs,mathtools,amsmath,amsthm,amssymb,amsfonts,stmaryrd,upgreek}
\usepackage{bbm,mathrsfs,mathtools,amsmath,amssymb,amsfonts,stmaryrd,upgreek}
%\usepackage{MnSymbol}
\usepackage{fancyhdr,subfigure}
%\usepackage[small,normal,bf,up]{caption}
\usepackage{epsfig,graphicx,wrapfig,fancyvrb,listings,color,textcomp,float}
%\usepackage[section]{algorithm}
%\usepackage{algorithmicx,algpseudocode}
%\usepackage{algorithmic}
\usepackage{algorithm}
\Crefname{ALC@unique}{Line}{Lines}
\usepackage{enumitem,url,hyperref}
%\usepackage[sort&compress]{natbib}
%\usepackage{sidecap,titlesec,scalerel}
%\sidecaptionvpos{figure}{c} % center the text
%\usepackage{ulem,subfig,fancyhdr}
%\usepackage[english]{babel}

\usepackage{tikz}
\usepackage{tikz-qtree}
\usetikzlibrary{positioning}
\usetikzlibrary{calc}

% Define basic notation
\newcommand{\state}{ {\mathbf{x}} }
\newcommand{\param}{ {\boldsymbol{\uptheta}} }
\newcommand{\Param}{ {\Theta} }
\newcommand{\adjoint}{ {\boldsymbol{\uplambda}} }
\newcommand{\obs}{ {\mathbf{Y}} }
\newcommand{\Obs}{ {Y} }
\newcommand{\sen}{ \mathbf{s} }
\newcommand{\Jfunc}{\Psi}                    % Cost function
\newcommand{\Jfuncd}{\Psi^\textrm{d}} % Discrete cost function
\newcommand{\nstate}{n}
\newcommand{\nparam}{p}
\newcommand{\nobs}{m}  % Dimension of observation vector
\newcommand{\ndata}{N} % Number of data points
\newcommand{\neqn}{q}
\newcommand{\nout}{ \textnormal{\tiny $\mathscr{O}$} }


\usepackage[listings,skins,breakable]{tcolorbox}
\newenvironment{popovnote}{\begingroup
\begin{tcolorbox}[breakable,enhanced jigsaw, colback=Fuchsia!20,colframe=black,title={\textsc{Andrey}}]%
}%
{%
\end{tcolorbox}\endgroup}

%%% Material that is not yet complete %%%%
\newif\ifcomplete


% Observations
\newcommand{\Hobs}{\mathcal{H}}
\newcommand{\HH}{\mathbf H}
\newcommand{\Nobs}{ {\rm N}_{\rm obs} }
\newcommand{\ObsOpL}{\mathbf{G}}  % Linear observation operator
\newcommand{\ObsOp}{\mathcal{G}}  % Nonlinear observation operator


% Matrices
\newcommand{\A}{ \mathbf{A} }
\newcommand{\B}{ \mathbf{B} }
\newcommand{\C}{\mathbf{C}}
\newcommand{\E}{\mathbf{E}}
\newcommand{\F}{\mathbf{F}}
\newcommand{\G}{\mathbf{G}}
\renewcommand{\H}{ \mathbf{H} }
\newcommand{\I}{ \mathbf{I} }
\newcommand{\J}{ \mathbf{J} }
\newcommand{\K}{ \mathbf{K} }
\renewcommand{\L}{ \mathbf{L} }
\newcommand{\V}{ \mathbf{V} }
\newcommand{\W}{ \mathbf{W} }
\newcommand{\Sen}{ \mathbf{S} }
\newcommand{\Z}{ \mathbf{Z} } 
\newcommand{\Zero}{\mathbf{0}}
\newcommand{\Id}{ \mathbf{I} }
\newcommand{\R}{ \mathbf{R} }
\renewcommand{\P}{\mathbf{P}}
\newcommand{\Pa}{\mathbf{P}^{\rm a}}
\newcommand{\Pb}{\mathbf{P}^{\mathrm{b}}}
%\newcommand{\SqrtPa}{\mathbf{P}^{{\rm a}\,1/2}}
%\newcommand{\SqrtPb}{\mathbf{P}^{{\mathrm{b}}\,1/2}}
\newcommand{\Pbl}{\mathbf{P}^{\rm b,loc}}
\usepackage{accents}
\newcommand*{\bigdot}[1]{\accentset{\mbox{\large\bfseries .}}{#1}}
\newcommand{\Sa}{\bigdot{\Xens}^{\rm a}}
\newcommand{\Sb}{\bigdot{\Xens}^{\mathrm{b}}}
\newcommand{\Pf}{\mathbf{P}^{\rm f}}
\newcommand{\Q}{\mathbf{Q}}
\newcommand{\bPi}{\boldsymbol\Pi}

% Operators
\newcommand{\Msolution}{ \mathcal{M} }
\newcommand{\Mequation}{ \mathcal{F} }
%\newcommand{\Model}{\mathcal{M}}
\newcommand{\M}{\mathbf{M}}
\newcommand{\Mtlm}{\mathbf{M}}
\newcommand{\Madj}{\mathbf{M}^*}

% Vectors
\newcommand{\x}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {X}
      {X^{[#1]}}}
      
\renewcommand{\u}{U}
\newcommand{\uh}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\hat{U}}
      {\hat{u}^{(#1)}}}
%\newcommand{\xb}[1][]{%
%   \ifthenelse{ \equal{#1}{} }
%      {\mathbf{x}^{\mathrm{b}}}
%      {\mathbf{x}^{{\mathrm{b}}[#1]}}}
\newcommand{\xb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {X^{\mathrm{b}}}
      {\mathbf{X}^{\mathrm{b},[#1]}}}
      
\newcommand{\ub}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {U^{\mathrm{b}}}
      {\mathbf{U}^{\mathrm{b},[#1]}}}
      
\newcommand{\ua}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {U^{\mathrm{a}}}
      {\mathbf{U}^{\mathrm{a},[#1]}}}
      
\newcommand{\uha}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\hat{U}^{\mathrm{a}}}
      {\mathbf{\hat{U}}^{\mathrm{a},[#1]}}}
      
\newcommand{\pub}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\*\Phi_r\,U^{\mathrm{b}}}
      {\*\Phi_r\,\mathbf{U}^{\mathrm{b},[#1]}}}
      
\newcommand{\uhb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\hat{U}^{\mathrm{b}}}
      {\mathbf{\hat{U}}^{\mathrm{b},[#1]}}}
      
\newcommand{\puhb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\*\Phi_r\,\hat{U}^{\mathrm{b}}}
      {\*\Phi_r\,\mathbf{\hat{U}}^{\mathrm{b},#1}}}
      
\newcommand{\zb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {Z^{\mathrm{b}}}
      {\mathbf{Z}^{\mathrm{b},#1}}}
      
\newcommand{\za}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {Z^{\mathrm{a}}}
      {\mathbf{Z}^{\mathrm{a},[#1]}}}
      
% \newcommand{\xa}[1][]{%
%   \ifthenelse{ \equal{#1}{} }
%       {\mathbf{x}^{\rm a}}
%       {\mathbf{x}^{{\rm a}[#1]}}}
\newcommand{\xa}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {X^{\rm a}}
      {\mathbf{X}^{\mathrm{a},[#1]}}}
\newcommand{\xf}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\mathbf{x}^{\rm f}}
      {\mathbf{x}^{{\rm f}[#1]}}}
\newcommand{\xt}{ \mathbf{X}^{\mathrm{t}} }
\newcommand{\xnat}{ \mathbf{x}^{\rm nature} }
\newcommand{\xv}{ \mathbf{x}^{\rm ver} }
\newcommand{\xmean}{ \overline{\mathbf{x}} }
\newcommand{\xmeanb}{ \overline{\mathbf{x}}^{\mathrm{b}} }
\newcommand{\xmeana}{ \overline{\mathbf{x}}^{\rm a} }
\newcommand{\hofx}{\mathbf{z}}
\newcommand{\hofxmeanb}{ \overline{\mathbf{z}}^{\mathrm{b}} }
\newcommand{\hofxmeana}{ \overline{\mathbf{z}}^{\rm a} }
\newcommand{\hofxb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\hofx^{\mathrm{b}}}
      {\hofx^{{\mathrm{b}}[#1]}}}
\newcommand{\hofxa}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\hofx^{\rm a}}
      {\hofx^{{\rm a}[#1]}}}
\newcommand{\dhofxb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\bigdot{\hofx}^{\mathrm{b}}}
      {\bigdot{\hofx}^{{\mathrm{b}}[#1]}}}
\newcommand{\y}{ \mathbf{y} }
\newcommand{\yini}{ \mathbf{y}_0 }
\newcommand{\ystage}{ \mathbf{Y} }
\newcommand{\z}{ \mathbf{z} }
\newcommand{\zstage}{ \mathbf{Z} }
\renewcommand{\v}{ \mathbf{v} }
\newcommand{\w}{ \mathbf{w} }
\renewcommand{\b}{ \mathbf{b} }
\newcommand{\f}{ \mathbf{f} }
\renewcommand{\k}{ \mathbf{k} }
\newcommand{\clambda}{ \overline{\lambda} }
\newcommand{\slambda}{ \lambda^\textrm{d} }
\newcommand{\cmu}{ \overline{\mu} }
\newcommand{\one}{\mathbf{1}}
\newcommand{\sv}{{\rm s}} % singular vector

% Errors
\newcommand{\errb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\varepsilon^{\mathrm{b}}}
      {\varepsilon^{{\mathrm{b}}[#1]}}}
\newcommand{\erra}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\varepsilon^{\rm a}}
      {\varepsilon^{{\rm a}[#1]}}}
%\newcommand{\erro}[1][]{%
%   \ifthenelse{ \equal{#1}{} }
%      {\varepsilon^{\rm o}}
%      {\varepsilon^{{\rm o}[#1]}}}
\newcommand{\erro}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\eta}
      {\boldsymbol{\eta}^{(#1)}}}
\newcommand{\biasa}{\beta^{\rm a} }
\newcommand{\errm}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {\eta}
      {\eta^{[#1]}}}
% Weights
\newcommand{\wb}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {w^{\mathrm{b}}}
      {w^{{\mathrm{b}}[#1]}}}
\newcommand{\wa}[1][]{%
   \ifthenelse{ \equal{#1}{} }
      {w^{\rm a}}
      {w^{{\rm a}[#1]}}}


% Times
\newcommand{\tb}{t_0}
\newcommand{\tf}{t_{\rm F}}
\newcommand{\tv}{t_{\rm v}}

% Spaces
\renewcommand{\Re}{\mathbbm{R}}
\newcommand{\Co}{\mathbbm{C}}
\newcommand{\Nat}{\mathbbm{N}}
\newcommand{\Leb}{\mathbbm{L}}
\newcommand{\Sob}{\mathbbm{H}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Y}{\mathcal{Y}}
\newcommand{\U}{\mathcal{U}}
\renewcommand{\H}{\mathcal{H}}
%
\newcommand{\Hstate}{\mathcal{H}_\state}
\newcommand{\Hparam}{\mathcal{H}_\param}
\newcommand{\Hmodel}{\mathcal{H}_\textrm{F}}


% Environments
%\newtheorem{definition}{Definition}
\newtheorem{problem}{Problem}
%\newtheorem{theorem}{Theorem}
\newtheorem{example}{Example}
%\newtheorem{comment}{Comment}
\newtheorem{remark}{Remark}
%\newtheorem{lemma}{Lemma}
\newtheorem{assumption}{Assumption}

% Probabilities
\newcommand{\Prob}{\mathcal{P}}
\newcommand{\PA}{ {\mathcal P}^{\rm a} }
\newcommand{\PB}{ {\mathcal P}^{\mathrm{b}} }
\newcommand{\PF}{ {\mathcal P}^{\rm f} }
\newcommand{\PO}{ {\mathcal P}^{\rm obs} }
\newcommand{\expect}[1]{\mathtt{E}\left[#1\right]}
\newcommand{\expectw}[2]{\mathtt{E}^{#1}\left[#2\right]}
\newcommand{\cov}[1]{\mathtt{Cov}\left[#1\right]}
\newcommand{\corr}[1]{\mathtt{Corr}\left[#1\right]}
\newcommand{\var}[1]{\mathtt{Var}\left[#1\right]}
\newcommand{\std}[1]{\mathtt{Std}\left[#1\right]}
\newcommand{\EnsA}{\mathtt{E}^{\rm a}}
\newcommand{\EnsB}{\mathtt{E}^{\mathrm{b}}}
\newcommand{\entropy}[1]{\mathtt{H}\left[#1\right]}
\newcommand{\from}{\sim}
\newcommand{\iidfrom}{\stackrel{\textnormal{i.i.d.}}{\sim}}

% Operations
\newcommand{\scalar}[1]{\left\langle\, #1 \,\right\rangle} 
\newcommand{\scalaralt}[1]{\left\lgroup\, #1 \,\right\rgroup} 
\newcommand{\norm}[1]{\bigl\Vert #1 \bigr\Vert} 
\newcommand{\duality}[1]{\left\llangle #1 \right\rrangle} 
\newcommand{\dualityalt}[1]{\left\llbracket #1 \right\rrbracket} 
\newcommand{\explain}[2]{\underset{#2}{\underbrace{#1}}}


% PDE notation
\renewcommand{\a}{\mathcal{N}}
\newcommand{\qq}{\mathbf{q}}
\newcommand{\dq}{ {\boldsymbol\psi}_{ \mathbf{\scriptscriptstyle q} } }
\newcommand{\bq}{ {\boldsymbol\phi}_{ \mathbf{\scriptscriptstyle q} } }
\newcommand{\uu}{\mathbf{u}}
\newcommand{\du}{ {\boldsymbol\psi}_{ \mathbf{\scriptscriptstyle u} } }
\newcommand{\bu}{ {\boldsymbol\phi}_{ \mathbf{\scriptscriptstyle u} } }
\newcommand{\llam}{ {\boldsymbol\lambda} }
\newcommand{\dl}{ {\boldsymbol\psi}_{ {\scriptscriptstyle \boldsymbol \lambda} } }
\newcommand{\bl}{ {\boldsymbol\phi}_{ {\scriptscriptstyle \boldsymbol \lambda} } }
\newcommand{\eu}{ \mathbf{e}_\uu }
\newcommand{\el}{ \mathbf{e}_{\llam} }
\newcommand{\eq}{ \mathbf{e}_\qq }
\newcommand{\zz}{ \mathbf{z} }
\newcommand{\ww}{ \mathbf{w} }
\newcommand{\vv}{ \mathbf{v} }
\newcommand{\bsigma}{ {\boldsymbol\sigma} }
\newcommand{\bdelta}{ {\boldsymbol\delta} }
\newcommand{\bxi}{ {\boldsymbol\xi} }
\newcommand{\bpsi}{ {\boldsymbol\psi} }
\newcommand{\bphi}{ {\boldsymbol\phi} }
\newcommand{\bchi}{ {\boldsymbol\chi} }
\newcommand{\ofbxi}{\left[{\boldsymbol\xi}\right]}
\newcommand{\ofbxiopt}{\left[{\boldsymbol\xi_*}\right]}
\newcommand{\brho}{ {\boldsymbol\rho} }


% EnKF
\newcommand{\Xens}{\mathbf{X}}
\newcommand{\Xensf}{\mathbf{X}^{\rm f}}
\newcommand{\Xensb}{\mathbf{X}^{\mathrm{b}}}
\newcommand{\Xensa}{\mathbf{X}^{\rm a}}
\newcommand{\hofXens}{\mathbf{Z}}
\newcommand{\hofXensb}{\mathbf{Z}^{\mathrm{b}}}
\newcommand{\hofXensa}{\mathbf{Z}^{\rm a}}
\newcommand{\Gb}{\bigdot{\mathbf{Z}}^{\mathrm{b}}}
\newcommand{\Ga}{\bigdot{\mathbf{Z}}^{\rm a}}
\newcommand{\Yens}{\mathbf{Y}}
\newcommand{\Info}{\mathcal{I}}
\newcommand{\Nens}{{{\rm N}}}
\newcommand{\Nstate}{{{\rm N}_{\rm state}}}

% ROM
\newcommand{\Nrom}{{{\rm N}_{\rm rom}}}

% Typesetting
\newcommand{\ditto}{---\;\raisebox{-0.7ex}{''}\,---}



==> Model Forest EnKF_1_sub/shared.tex <==
%\usepackage[utf8]{inputenc}
\usepackage{cite}[sort]

\usepackage{tkz-graph}

\usetikzlibrary{calc}

\usepackage{pgfplots}

\pgfplotsset{compat=1.16}

\newcommand{\creflastconjunction}{, and~}


\input{header.tex}


%\renewcommand{\thesection}{\arabic{section}}
%\renewcommand{\thesubsection}{\thesection.\arabic{subsection}}
%\renewcommand{\thesubsubsection}{\thesubsection.\arabic{subsubsection}}
%\makeatletter
%\renewcommand{\p@subsection}{}
%\renewcommand{\p@subsubsection}{}
%\makeatother

\input{usefulstuff.tex}

% colors
\newcommand{\red}[1]{{\color{red}\{(Andrey) #1\}}}
\newcommand{\sandu}[1]{{\color{purple}\{(Sandu) #1\}}}

\DeclareMathOperator{\diag}{diag}

\graphicspath{ {Figures/} }


\def\realtitle{The Model Forest Ensemble Kalman Filter}


\title{{\realtitle}\thanks{Submitted to the ArXiv \today.
		\funding{The work of Popov and Sandu was supported by DOE through award ASCR DE-SC0021313, by NSF  through award  CDS\&E--MSS 1953113, and by the Computational Science Laboratory at Virginia Tech.}}}
\date{\today}
%\author{Andrey A. Popov\thanks{Oden Institute for Computational Engineering and Sciences, University of Texas at Austin, Austin, TX (\email{andrey.a.popov@utexas.edu})}\textsuperscript{, }\footnotemark[2]
%\and Adrian Sandu\thanks{Computational Science Laboratory, Department of Computer Science, Virginia Tech, Blacksburg, VA   (\email{sandu@cs.vt.edu}).}
%}


\author{Andrey A. Popov\textsuperscript{, }\footnotemark[2]\ \footnotemark[3]
\and Adrian Sandu\footnotemark[3]
}




\tikzset{MainModel/.style={circle, draw=red!85, fill=red!5, very thick, minimum size=22mm},
    SurrModel/.style={circle, draw=RoyalBlue!85, fill=RoyalBlue!5, thick, minimum size=16mm},
    MainModelSmall/.style={circle, draw=red!85, fill=red!5, thick, minimum size=0.5em, inner sep=0pt}, 
    SurrModelSmall/.style={circle, draw=RoyalBlue!85, fill=RoyalBlue!5, semithick, minimum size=0.3em, inner sep=0pt},
    MainModelMedium/.style={circle, draw=red!85, fill=red!5, very thick, minimum size=7.33mm},
    SurrModelMedium/.style={circle, draw=RoyalBlue!85, fill=RoyalBlue!5, thick, minimum size=5.33mm},}

\tikzset{MainModel/.style={circle, draw=red!85, fill=red!5, very thick, minimum size=22mm},
    SurrModel/.style={circle, draw=RoyalBlue!85, fill=RoyalBlue!5, thick, minimum size=16mm},
    MainModelSmall/.style={circle, draw=red!85, fill=red!5, thick, minimum size=0.5em, inner sep=0pt}, 
    SurrModelSmall/.style={circle, draw=RoyalBlue!85, fill=RoyalBlue!5, semithick, minimum size=0.3em, inner sep=0pt}}

\newcommand{\mainmodel}{\raisebox{0em}{\begin{tikzpicture}
            \node[MainModelSmall] (t1root) at (0,0) {};
\end{tikzpicture}}}


\newcommand{\surrmodel}{\raisebox{0em}{\begin{tikzpicture}
            \node[SurrModelSmall] (t1root) at (0,0) {};
\end{tikzpicture}}}

\newcommand{\modelaverage}{\raisebox{0em}{\begin{tikzpicture}
            \node[MainModelSmall] (t1root) at (0,0) {};
            \node[MainModelSmall] (t2root) at (1.35em,0) {};
            \draw[very thick, dotted] (t1root) -- (t2root);
\end{tikzpicture}}}


\newcommand{\treeonesurr}{\raisebox{-0.28em}{\begin{tikzpicture}
            \node[MainModelSmall] (t1root) at (0,0) {};
            \node[SurrModelSmall] (t1sur1) at (0,-0.6em) {};
            \draw[very thick] (t1root) -- (t1sur1);
\end{tikzpicture}}}

\newcommand{\treetwosurr}{\raisebox{-0.28em}{\begin{tikzpicture}
            \node[MainModelSmall] (t1root) at (0,0) {};
            \node[SurrModelSmall] (t1sur1) at (-0.5em,-0.5em) {};
            \node[SurrModelSmall] (t1sur2) at (0.5em,-0.5em) {};
            \draw[very thick] (t1root) -- (t1sur1);
            \draw[very thick] (t1root) -- (t1sur2);
\end{tikzpicture}}}

\newcommand{\forestonesurr}{\raisebox{-0.28em}{\begin{tikzpicture}
            \node[MainModelSmall] (t1root) at (0,0) {};
            \node[SurrModelSmall] (t1sur1) at (0,-0.6em) {};
            \draw[very thick] (t1root) -- (t1sur1);
            
            \node[MainModelSmall] (t2root) at (1.35em,0) {};
            \node[SurrModelSmall] (t2sur1) at (1.35em,-0.6em) {};
            \draw[very thick] (t2root) -- (t2sur1);
            
            \draw[very thick, dotted] (t1root) -- (t2root);
\end{tikzpicture}}}







==> Model Forest EnKF_1_sub/usefulstuff.tex <==
\newcommand\1{\one}
\def\!#1{\mathcal{#1}}
\def\*#1{\boldsymbol{\mathbf{#1}}}
\def\|#1{\textnormal{#1}}

\def\det#1{\left\lvert#1\right\rvert}
\def\norm#1{\left\lVert#1\right\rVert}
\def\diff#1{\mathrm{d}#1}
\def\sgn{\text{sgn}}

\newcommand{\Mean}[1]{\*\mu_{#1}}
\newcommand{\MeanE}[1]{\widetilde{\*\mu}_{#1}}
\newcommand{\Cov}[2]{\*\Sigma_{#1,#2}}
\newcommand{\Covs}[1]{\*\Sigma_{#1}}
\newcommand{\CovE}[2]{\widetilde{\*\Sigma}_{#1,#2}}
\newcommand{\KE}[1]{\widetilde{\*\K}_{#1}}
\newcommand{\En}[1]{\mathsf{E}_{#1}}
\newcommand{\An}[1]{\mathsf{A}_{#1}}
\renewcommand{\Z}[2][\Hobs_i]{\mathsf{A}_{#1(#2)}}

\DeclareMathOperator*{\argmin}{arg\,min}
\newcommand{\inner}[2]{\left\langle#1,#2\right\rangle}

\DeclareMathOperator{\tr}{tr}

% specific model stuff
\newcommand{\Model}[1]{\mathcal{M}^{#1}}




\def\TK#1{{\color{red}#1}}

\newenvironment{tk}
    {\color{red}
    }
    {}
